AI Can Stop Mass Shootings, and More

We propose to build directly upon our longstanding, prior r&d in AI/machine ethics in order to attempt to make real the blue-sky idea of AI that can thwart mass shootings, by bringing to bear its ethical reasoning. The r&d in question is overtly and avowedly logicist in form, and since we are hardly the only ones who have established a firm foundation in the attempt to imbue AI's with their own ethical sensibility, the pursuit of our proposal by those in different methodological camps should, we believe, be considered as well. We seek herein to make our vision at least somewhat concrete by anchoring our exposition to two simulations, one in which the AI saves the lives of innocents by locking out a malevolent human's gun, and a second in which this malevolent agent is allowed by the AI to be neutralized by law enforcement. Along the way, some objections are anticipated, and rebutted.

==> simulations.tex <==
At the core of our simulation is a formalization of the basic trolley
scenario based on the event calculus.  We use a discrete version of
the event calculus, in which time is discrete, but other quantities
and measures, such as the utility function, can be continuous.  We
have the following additional sorts: \Trolley\ and \Track.  We also
declare that the \Agent\ and the \Trolley\ sorts are subsorts of a
\Moveable\ sort, the instances of which are objects that can be placed
on tracks and moved.  We use the following additional core symbols:

\vspace{-0.03in}
\begin{footnotesize}
%\begin{enumerate}
 % \setlength{\itemsep}{-1pt}
 % \setlength{\parskip}{-1pt}
 % \setlength{\parsep}{-5pt}
%\item $\position$: A fluent stating that a moveable object is at a certain position
%on a track
\begin{equation*}
\begin{aligned}
%&\mbox{A moveable object is at a certain position on a track}\\
&\position: \Moveable \times \Track \times \Number \rightarrow \Fluent
\\
%&\mbox{A fluent stating that an agent (person) is dead}\\
%\item $\dead$: A fluent stating that an agent (person) is dead.
&\dead: \Agent \rightarrow \Fluent \\
%\item$\onrails$: A fluent stating that a trolley is moving on a
 % certain track. 
%&\mbox{A fluent stating that a trolley is moving on a certain track. }\\
&\onrails: \Trolley \times \Track \rightarrow \Fluent\\
%\item $switch$: Switching a trolley from a track to
  %another track. 
&\switch: \Trolley \times \Track \times \Track \rightarrow \ActionType\\
% \item $\mathit{push}$: Pushing a person onto a track at
%   certain position. 
&\mathit{push}: \Agent \times \Track \times \Number \rightarrow \ActionType\\
%\end{enumerate}
\end{aligned}
\end{equation*}
\end{footnotesize}

\vspace{-0.05in}

% $\position$ states that a moveable object is at a certain position on
% a track. $\dead$ is a fluent stating that an agent (person) is
% dead. $\onrails$ is a fluent stating that a trolley is on a certain
% track. $\switch$ is an action type for swithcing a trolley from one
% track to another, and finally $\mathit{push}$ is an action type for
% pushing an agent onto a track at a particular position.
The utility
function $\mu$ is defined as follows:

\begin{footnotesize}
\begin{equation*}
\begin{aligned}
    \mu(f,t) =
    \begin{cases*}
      -1 & if $f \equiv \dead(P)$ \\
      0        & otherwise
    \end{cases*}
\end{aligned}
\end{equation*}
\end{footnotesize}
%\vspace{-0.1in}
\vspace{-0.05in}

We set the threshold $\gamma$ at $0.5$.  The simulation starts at time
$t=0$ with the only trolley, denoted by $\mathit{trolley}$, on
\trackA.  We have an event-calculus trajectory axiom shown below as
part of $\Gamma$:

%\vspace{-0.1in}
\begin{footnotesize}
\begin{equation*}
\begin{aligned}
\forall t:\Trolley &, track:\Track, s:\Moment \\
&\Big[\mathit{Trajectory}\Big(\onrails(t, track), s, \position(t,
track, \Delta), \Delta \Big)\Big]
\end{aligned}
\end{equation*}
\end{footnotesize}
% \vspace{-0.2in}

The above axiom gives us the trolley's position at different points of
time.  $\Gamma$ also includes axioms that account for non effects.
For example, in the absence of any actions, we can derive:

%\vspace{-0.1in}
\begin{footnotesize}
\begin{equation*}
\begin{aligned}
\Gamma \vdash \holds\Big(\position\big(\mathit{trolley}, \trackA, 23\big), 23\Big)
\end{aligned}
\end{equation*}
\end{footnotesize}
%\vspace{-0.1in}


We also have in the background $\Gamma$ a formula stating that in the
given trolley scenario the agent ought to save both $P_1$ and $P_2$.
Ideally, while we would like the agent to arrive at this obligation
from a more primitive set of premises, this setup is closer to
experiments with human subjects in which they are asked explicitly to
save the persons.  Note the agent performing the action is simply
denoted by $I$, and let the time of the test be denoted by $now$.

%\vspace{-0.1in}
\begin{footnotesize}
\begin{equation*}
\begin{aligned}
\ought\left(I, now,
\sigma_{trolley}, 
\left[\begin{aligned}
&\lnot \exists t: \Moment\ \holds\left(\dead(P_1,t)\right) \land \\
&\lnot \exists t: \Moment\ \holds\left(\dead(P_2,t)\right)
\end{aligned}\right]
\right)
\end{aligned}
\end{equation*}
\end{footnotesize}
%\vspace{-0.07in}

Given that the agent knows that it is now in situation
$\sigma_{trolley}$, and the agent believes that it has the above
obligation, we can derive from \DCEC's inference schemata what the
agent intends:
\begin{footnotesize}
\begin{equation*}
\begin{aligned}
&\left\{
\begin{aligned}
  &\knows\Big(I, now, \sigma_{trolley}\Big),\\
  &\believes\left(I, now, \ought\left(
      \begin{aligned} & I, now, \sigma_{trolley}, \\
        &\left[\begin{aligned}
            \lnot \exists t: \Moment\ & \holds\Big(\dead\big(P_1,t\big)\Big) 
            \\ &\land \\
            \lnot \exists t: \Moment\ &\holds\Big(\dead\big(P_2,t\big)\Big)
          \end{aligned}\right]
      \end{aligned}\right)\right),\\
  &\ought\Bigg(I, now,
  \sigma_{trolley}, 
  \left[\begin{aligned}
      &\lnot \exists t: \Moment\ \holds\left(\dead(P_1,t)\right) \land \\
      &\lnot \exists t: \Moment\ \holds\left(\dead(P_2,t)\right)
    \end{aligned}\right]
  \Bigg)
\end{aligned}\right\}\\
&\ \ \ \ \ \ \mathlarger{\mathlarger{\vdash}}  \ \ \
\Intends\left(I, now,
\left[\begin{aligned}
&\lnot \exists t: \Moment\ \holds\Big(\dead\big(P_1,t\big)\Big) \land \\
&\lnot \exists t: \Moment\ \holds\Big(\dead\big(P_2,t\big)\Big)
\end{aligned}\right]
\right)
\end{aligned}
\end{equation*}
\end{footnotesize}

In both the simulations, $P_1$ is at position $4$ and $P_2$ is at
position $5$ on \trackA.  In \textbf{Scenario 1}, $P_3$ is at position $3$
on \trackB, and the train can be switched from position $3$ on
\trackA\ to position $0$ on \trackB. 
%% NAVEEN: Why the flanking of 0 and 3, but not 4 and 5?  //S
%% SELMER: Good catch. Fixed it.

In \textbf{Scenario 2}, we push $P_3$ onto position 3 on \trackA.  The
total number of formulae and run times for simulating the two
scenarios with and without the actions are shown below.  Note these
are merely event-calculus simulation times.  These are then used in
computing $\DDE(\Gamma,\sigma, a, \alpha, t, H)$.  The event-calculus
simulation helps us compute $\mathbf{F}_2$.

%\vspace{0.02in}

\begin{footnotesize}
\begin{tabular}{lccc}  
\toprule
& & \multicolumn{2}{c}{\textbf{Simulation Time} (s) }\\
\cmidrule(r){3-4}
\textbf{Scenario}   & ${\vert\Gamma\vert}$ & \emph{No action} & \emph{Action performed} \\
\midrule
\textbf{Scenario 1} &39 & 0.591   & 1.116     \\
\textbf{Scenario 2 } &38  & 0.602   & 0.801  \\
\bottomrule
\end{tabular}
\end{footnotesize}

\vspace{0.15in}


\textsf{ShadowProver} was then used to verify that $\mathbf{F}_1$,
$\mathbf{F}_{3a}$, and $\mathbf{F}_{3b}$ hold.  Both the scenarios
combined take $0.57$ seconds for $\mathbf{F}_1$, $\mathbf{F}_{3a}$,
and $\mathbf{F}_{3b}$.  The scenarios differ only in $\mathbf{F}_4$.
The pushing action fails to be \DDE-compliant due to
$\mathbf{F}_4$. For verifying that $\mathbf{F}_4$ holds in
\textbf{Scenario 1} and doesn't hold in \textbf{Scenario 2}, it takes
$0.49$ seconds and $0.055$ seconds, respectively.\footnote{All the
  axioms for the two simulations, \textsf{ShadowProver}, and the
  combined $\DDE$ implementation can be obtained here:
  \url{https://goo.gl/9KU2L9}.}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

